Bounded Control for Double Integrator in Quadrotor Dynamics

We construct a trajectory tracking controller for a quadrotor system by finding a coordinate change which transforms the quadrotor's vector field into that of a thrust propelled system. In a thrust propelled system, the goal is to stabilize its position around the origin, while the system is actuated by a one dimensional acceleration/thrust along a direction vector, by a time-varying gravity, and by the angular acceleration of the direction vector. For this system, a solution has been proposed in a companion article, submitted to ECC 2016, based on the implicit knowledge of a bounded controller for a double integrator system, and on the implicit knowledge of a Lyapunov function that guarantees the origin is asymptotically stable for the double integrator controlled by the bounded controller. We present two alternative bounded controllers for a double integrator system, and corresponding Lyapunov functions.

==> Contents/FullyActuated.tex <==
We now consider the case when $k_{\sss{T}} $ is not perfectly known. 
%
For this scenario, we denote $\hat{k}_{\sss{T}}$ as a disturbance estimate and 
%
\begin{align}
	\dot{\hat{k}}_{\sss{T}}(t)
	=
	f_{\sss{k}}(t,\xmb,\hat{k}_{\sss{T}}(t)),
\end{align}
%
where $f_{\sss{k}}(t,\xmb,\hat{k}_{\sss{T}})$ is a function to be designed such that the goal of Problem~\ref{prob:Problem} is still accomplished.
%

By looking at~\eqref{eq:f1}-\eqref{eq:f3}, a natural solution to the problem is to modify $T(t)$ as
%
\begin{align}
	T(t) 
	=
	\frac{\mQ}{\hat{k}_{\sss{T}}}
	T_{\sss{cl}}(t,\bar{\xmb}(t)),
	\label{eq:ThrustDisturbance}
\end{align}
%
because, if  $\hat{k}_{\sss{T}}(t) = k_{\sss{T}}$ for all $t \ge 0$, then the results from the previous section apply.

For convenience, denote $\tilde{k}(t) = k_{\sss{T}} - \hat{k}_{\sss{T}}(t)$, and $\xmb^{\sss{e}} = [\xmb\tp \, \hat{k}_{\sss{T}}]\tp$. 
%
Then, if the thrust is chosen as in~\eqref{eq:ThrustDisturbance}, it follows that $\dot{\xmb}^{\sss{e}}(t) = [\fmb_{\sss{d}}\tp(t,\xmb(t),\hat{\bmb}(t)) \, f_{\sss{k}}(t,\xmb(t),\hat{k}_{\sss{T}})]\tp := \fmb^{\sss{e}}(t,\xmb^{\sss{e}}(t))$, where
%
\begin{align}
	\fmb_{\sss{d}}(t,\xmb,\hat{\bmb})
	& =
	\fmb_{\sss{u}}^{\sss{cl}}(t,\xmb)
	+
	\begin{bmatrix}
		\zvec_{\sss{3}}
		\\
		\frac{k - \hat{k}_{\sss{T}}}{\hat{k}_{\sss{T}}} \frac{T_{\sss{cl}(t,\bar{\xmb}(t))}}{\mQ} \rQ
		\\
		\zvec_{\sss{9}}
	\end{bmatrix}	
	\\
	&
	:=
	\fmb_{\sss{u}}^{\sss{cl}}(t,\xmb)
	+
	\Phi(\xmb^{\sss{e}}) (k - \hat{k}_{\sss{T}})		
\end{align}

The vector field  $f_{\sss{k}}(t,\xmb,\hat{k}_{\sss{T}})$ can now be designed by considering the functions $V_{\sss{k}}(s) = \frac{1}{k_{\sss{i}}}\frac{s^2}{2}$, and
%
\begin{align}
	V(t,\xmb^{\sss{e}}) = V_{\sss{3}}(t,\xmb) + V_{\sss{k}}(k - \hat{k}_{\sss{T}}).
\end{align}

For the later function it follows that if 
%
\begin{align}
	f_{\sss{k}}(t,\xmb,\hat{k}_{\sss{T}})	= 
	\text{Proj}
	\left(
		k_{\sss{i}}\frac{\partial V\tp(t,\xmb)}{\partial \xmb} \Phi(\xmb^{\sss{e}})
		,
		\hat{k}_{\sss{T}}
	\right)
\end{align}
%
then
%
\begin{align}
	 & \frac{\partial V(t,\xmb^{\sss{e}})}{\partial t}
	+
	\frac{\partial V\tp(t,\xmb^{\sss{e}})}{\partial \xmb^{\sss{e}}}
	\fmb^{\sss{e}}(t,\xmb^{\sss{e}})
	=
	\\
	= &
	- W_{\sss{3}}(t,\xmb)
	-
	\\
	& 
	\frac{1}{k_{\sss{i}}}
	(k - \hat{k}_{\sss{T}})
	\left(
		f_{\sss{k}}(t,\xmb,\hat{k}_{\sss{T}})	 - k_{\sss{i}} \frac{\partial V_{\sss{3}}\tp(t,\xmb)}{\partial \xmb} \Phi(\zmb)
	\right),
	\\
	= : &
	-W(t,\xmb^{\sss{e}}) \le  - W_{\sss{3}}(t,\xmb) \le 0,
\end{align}
%
and, along a trajectory $\xmb^{\sss{e}}(t) $ for $\dot{\xmb}^{\sss{e}}(t) = \fmb^{\sss{e}}(t,\xmb^{\sss{e}}(t))$, $\dot{V}(t,\xmb^{\sss{e}}(t)) = - W(t,\xmb^{\sss{e}}(t)) \le - W_{\sss{3}}(t,\xmb(t))  \le 0$.



==> Contents/Simulations.tex <==
\begin{figure*}
	\centering	
	\subfigure[Trajectories]{
		\includegraphics[clip=true,trim=0cm 0cm 0cm 0cm,width=0.25\textwidth]{./Figures/Trajectory}
		\label{fig:Trajectory}
	}
	\subfigure[Position $\pmb$]{
		\includegraphics[clip=true,trim=0cm 0cm 0cm 0cm,width=0.25\textwidth]{./Figures/Position}
		\label{fig:Position}
	}
	\subfigure[Velocity $\vmb$]{
		\includegraphics[clip=true,trim=0cm 0cm 0cm 0cm,width=0.25\textwidth]{./Figures/Velocity}
		\label{fig:Velocity}
	}
	\subfigure[Unit vectors $\nmb$ in state and $\nmb_{\sss{t}}^{\sss{\star}}$ in~\eqref{eq:nStarEquilibrium}]{
		\includegraphics[clip=true,trim=0cm 0cm 0cm 0cm,width=0.25\textwidth]{./Figures/UnitVector}
		\label{fig:UnitVector}
	}	
	\subfigure[Angular velocities $\bm{\omega}$ in state and $\bm{\omega}^{\sss{d}}(t,\bar{\xmb}(t))$ in~\eqref{eq:OmegaD}]{
		\includegraphics[clip=true,trim=0cm 0cm 0cm 0cm,width=0.25\textwidth]{./Figures/AngularVelocities}
		\label{fig:AngularVelocities}
	}			
	\subfigure[Inputs $T(t) = T_{\sss{cl}}(t,\bar{\xmb}(t))$ and $\bm{\tau}(t) = \bm{\tau}_{\sss{cl}}(t,\xmb(t))$]{
		\includegraphics[clip=true,trim=0cm 0cm 0cm 0cm,width=0.25\textwidth]{./Figures/Inputs}
		\label{fig:Inputs}
	}	
\end{figure*}


==> Contents/SubActuated_Conflict_.tex <==
In this section, we assume that no disturbance is being exerted on the system~\ref{eq:f1}-\eqref{eq:f3}, i.e.,  $\bmb = \zvec$, and we design $T(t)$ and $\wQ(t)$ such that the goal of Problem~\ref{prob:QuadOmega} is accomplished.

In addition to $\nmb(t)$ $\wL(t)$, defined in~\eqref{eq:CableDirection} and~\eqref{eq:omega} respectively, let us also now define the variables
%
\begin{align}
	&\pmb(t) := \pL(t) - \pLstar(t)
	\\
	&\vmb(t) := \vL(t) - \vLstar(t)	
	\\
	&
	\gmb(t)
	:= 
	g\embThree + \aLstar(t),
\end{align} 
%
and, where the goal of Problem~\ref{prob:QuadOmega} is that $\lim_{\sss{t \rightarrow \infty}} \pmb(t) = \zvec$.
%
We also denote
%
\begin{align}
	%
	\xmb\tp
	:=	
	\begin{bmatrix}
		\bar{\xmb}\tp
		& 
		\bm{\omega}\tp
	\end{bmatrix}	
	:=		
	\begin{bmatrix}
		[\pmb\tp
		&
		\vmb\tp
		&
		\nmb\tp
		]
		&
		\bm{\omega}\tp
	\end{bmatrix}.
	\label{eq:stateQuad}
\end{align}
%
and
\begin{align}
	%
	\xmb^{\sss{e}}
	:=	
	\begin{bmatrix}
		\xmb\tp
		& 
		\rQ\tp
	\end{bmatrix}\tp.
	\label{eq:stateExtendedQuad}
\end{align}

For convenience, let us define
%
\begin{align}
	\umb(\xmb,\TensionStar,\TauCable)
	:=
	\nmb
	\left(
		(\mQ + \mL)\TensionStar - m d \|\wL\|^{\sss{2}} 
	\right)
	+
	\mQ \Length \TauCable,
	\label{eq:umb}
\end{align}
%
where $\nmb\tp\TauCable = 0$.
%
$\umb$ represents a force that along the cable direction has magnitude $\nmb\tp\umb = (\mQ + \mL)\TensionStar - m d \wL\tp\wL$, where $\TensionStar$ is to be constructed later and it is related to the tension that will be exerted on the cable; and along the plane orthogonal to the cable direction $\umb$ has magnitude $\OP{\nmb}\umb  = \mQ \Length \TauCable$, where $\TauCable $ is also to be defined later and it related to the angular acceleration of the cable.

Let us then choose the thrust $T(t)$ be of the form
%
\begin{align}
	T(t)
	& =
	\frac{\nmb\tp(t) \umb(\xmb(t),\TensionStar(t),\TauCable(t))}{\rQ\tp(t)\nmb(t)}
	\\
	& =
	\frac{1}{\rQ\tp(t)\nmb(t)} 
	\left(
		(\mQ + \mL)\TensionStar(t) - m d \|\wL(t)\|^{\sss{2}} 
	\right),
	\label{eq:Thrust}
\end{align}
%
where we assume that $\rQ\tp(t)\nmb(t) \ne 0$ for all time $t \ge 0$, and we give conditions when this satisfied later.
%
For this choice of thrust, it follows that the tension in the cable $\Tension(t)$ becomes (recall that $\bmb = \zvec$)
%
\begin{align}
	\Tension(t)
	\overset{\sss{\eqref{eq:Tension},\eqref{eq:Thrust}}}{=}
	\mL \TensionStar(t),
	\label{eq:TensionFinalQuad}
\end{align}
%
while the angular acceleration of the cable $\bm{\tau}(t)$  becomes
%
\begin{align}
	&
	\bm{\tau}(t)
	\overset{\sss{\eqref{eq:tau}}}{=}
	\frac{1}{\mQ \Length} \OP{\nmb(t)} \left(T(t) \rQ(t)	-  \umb(\cdot,\cdot,\cdot) + \umb(\cdot,\cdot,\cdot) \right)
	\\
	&
	\overset{\sss{\eqref{eq:umb}}}{=}
	\TauCable(t)
	+
	\frac{1}{\mQ \Length} \OP{\nmb(t)} \left(T(t) \rQ(t)	-  \umb(\cdot,\cdot,\cdot)	 \right)
	\\
	&
	\overset{\sss{\eqref{eq:Thrust}}}{=}
	\TauCable(t)
	+
	\frac{1}{\mQ \Length} \OP{\nmb(t)} \left( \frac{\rQ(t) \nmb\tp(t) }{\rQ\tp(t)\nmb(t)} -  \Idmat \right) \umb(\cdot,\cdot,\cdot)
%	\\
%	&
%	=
%	\TauCable(t)
%	+
%	\frac{1}{\mQ \Length \rQ\tp(t)\nmb(t)} \OP{\nmb(t)} \left( \rQ(t) \nmb\tp(t) -  \rQ\tp(t)\nmb(t) \Idmat \right) \umb(t)	
%	=
	\\
	&
	=
	\TauCable(t)
	+
	\frac{1}{\mQ \Length \rQ\tp(t)\nmb(t)} \OP{\nmb(t)}  \sk{\nmb(t) } \sk{\rQ(t)} \umb(\cdot,\cdot,\cdot)		
	\\
	& =
	\TauCable(t)
	+
	\frac{1}{\mQ \Length \rQ\tp(t)\nmb(t)} \OP{\nmb(t)}  \sk{\nmb(t) } \sk{\rQ(t)} \umb(\cdot,\cdot,\cdot)		
	\\
	& =
	\TauCable(t)
	+
	\frac{1}{\mQ \Length \rQ\tp(t)\nmb(t)} \sk{\nmb(t) } \sk{\rQ(t)}  \umb(\xmb(t),\TensionStar(t),\TauCable(t))
	\\
	& =:
	\TauCable(t)
	+
	\emb_{\sss{\theta}}(\xmb^{\sss{e}}(t),\TensionStar(t),\TauCable(t)).
	\label{eq:tauFinalQuad}
\end{align}
%

Notice now that if $T(t) \rQ(t) = \umb(\xmb(t),\TensionStar(t),\TauCable(t))$ (which can not be accomplished since  $\rmb(t)$ is not a control input), then $\emb_{\sss{\theta}}(\xmb^{\sss{e}}(t),\TensionStar(t),\TauCable(t)) = \zvec$ (if $\umb= \zvec$ the conclusions follows immediately, and if $\umb\ne \zvec$, then $T \rQ = \umb \Rightarrow \rQ = \frac{\umb}{\|\umb\|} \Rightarrow \sk{\rQ} \umb = \zvec$).
%
Thus if $T(t) \rQ(t) = \umb(\xmb(t),\TensionStar(t),\TauCable(t))$, then $\Tension(t) = \mL \TensionStar(t)$ and $\bm{\tau}(t) = \TauCable(t)$. 
%
If, however, $T(t) \rQ(t) \ne \umb(\xmb(t),\TensionStar(t),\TauCable(t))$, then $\bm{\tau}(t)$ will be $\TauCable(t)$ apart from an error $\emb_{\sss{\theta}}(\xmb^{\sss{e}}(t),\TensionStar(t),\TauCable(t))$ that vanishes if $\rQ(t)$ is aligned with the direction of $\umb(t)$.
%
This error is going to be propagated in a backstepping procedure.

From~\eqref{eq:f1}-\eqref{eq:f3} and \eqref{eq:nDot}-\eqref{eq:OmegaDot} it follows that if the thrust is selected as in~\eqref{eq:Thrust}, then
%
\begin{align}
	&\dot{\pmb}(t) = \vL(t)
	\\
	&\dot{\vmb}(t) 
	=  
	\frac{\Tension(t)}{\mL} \nmb(t) 
	-
	\gmb(t)
	\overset{\sss{\eqref{eq:TensionFinalQuad}}}{=}
	\TensionStar(t)\nmb(t) 
	-
	\gmb(t)
	\\
	&
	\dot{\nmb}(t)
	=\sk{\bm{\omega}(t)}
	\nmb(t)
	\\
	&
	\dot{\wL}(t)
	\overset{\sss{\eqref{eq:tauFinalQuad}}}{=} 
	\sk{\nmb(t)} \TauCable(t) + \emb_{\sss{\theta}}(\xmb^{\sss{e}}(t),\TensionStar(t),\TauCable(t)),
	\\
	&
	\rQDot(t)
	=
	\sk{\RQ(t)\wQ(t)} \rQ(t)
\end{align}

We can then write the dynamics of system as $\dot{\xmb}^{\sss{e}}(t) = \fmb(t,\xmb^{\sss{e}}(t),\TensionStar(t),\TauCable(t),\wQ)$, where
%
\begin{align}		
	\fmb(t,\xmb^{\sss{e}},\TensionStar,\TauCable,\wQ)
	& :=
	\begin{bmatrix}
			\vmb
			\\
			\TensionStar \nmb - \gmb(t)
			\\
			\sk{\bm{\omega}}\nmb
			\\
			\sk{\nmb} \TauCable
			\\
			\zvec
	\end{bmatrix}
	+
	\begin{bmatrix}
			\zvec
			\\
			\zvec
			\\
			\zvec
			\\
			\emb_{\sss{\theta}}(\xmb^{\sss{e}},\TensionStar,\TauCable)
			\\
			\sk{\RQ(t)\wQ} \rQ
	\end{bmatrix}	
	\\
	& :=
	\begin{bmatrix}
		\fmb_{\sss{u}}(t,\xmb,\TensionStar,\TauCable)
		\\
		\zvec
	\end{bmatrix}		
	+
	\begin{bmatrix}
		\zvec
		\\
		\sk{\nmb} \emb_{\sss{\theta}}(\xmb^{\sss{e}},\TensionStar,\TauCable)
		\\
		\sk{\RQ(t)\wQ} \rQ
	\end{bmatrix}	
\end{align}
%

The vector field $\fmb_{\sss{u}}(t,\xmb,\TensionStar,\TauCable)$ is that of a vector thrusted system, and a general solution that guarantees $\lim_{\sss{t \rightarrow \infty}} \pmb(t) = \zvec$ for $\dot{\xmb}(t) = \fmb_{\sss{u}}(t,\xmb(t),\TensionStar(t),\TauCable(t))$ can be found in~\cite{}.

In~\cite{}, we can find functions $T_{\sss{cl}}(t,\bar{\xmb})$  and $\bm{\tau}_{\sss{cl}}(t,\xmb)$ such that $\dot{\xmb}(t) = \fmb_{\sss{u}}^{\sss{cl}}(t,\xmb(t))$ where
%
\begin{align}
	\fmb_{\sss{u}}^{\sss{cl}}(t,\xmb) := \fmb_{\sss{u}}(t,\xmb,T_{\sss{cl}}(t,\bar{\xmb}),\bm{\tau}_{\sss{cl}}(t,\xmb))
\end{align}
%
it follows that $\lim_{\sss{t \rightarrow \infty}} \pmb(t) = \zvec$.
%
Also, for 
%
\begin{align}
	V_{\sss{3}}(t,\xmb)
	=
	V_{\sss{1}}(\pmb,\vmb)
	+
	V_{\sss{\theta}}(\xi(t,\bar{\xmb}))
	+
	V_{\sss{\omega}}(\emb_{\sss{\omega}}(t,\xmb)),
	\label{eq:V3}
\end{align}
%
the following is satisfied
%
\begin{align}
	 & \frac{\partial V_{\sss{3}}(t,\xmb)}{\partial t}
	+
	\frac{\partial V_{\sss{3}}(t,\xmb)}{\partial \xmb}
	\fmb_{\sss{u}}^{\sss{cl}}(t,\xmb(t))
	=
	\\
	= &
	-
	W_{\sss{1}}(\pmb,\vmb)
	-
	2
	k_{\sss{\omega}}
    V_{\sss{\omega}}(\emb_{\sss{\omega}}(t,\xmb))
    \\
    &
   	-
   	k_{\sss{\theta}}
   	V'_{\sss{\theta}}(\xi(t,\bar{\xmb}))
   	\xi(t,\bar{\xmb}) (2 - \xi(t,\bar{\xmb}))
	\\
	=: &
	- W_{\sss{3}}(t,\xmb) \le 0,
	\label{eq:W3}
\end{align}
%
and, along a trajectory $\xmb(t)$ with $\dot{\xmb}(t) = \fmb_{\sss{u}}^{\sss{cl}}(t,\xmb(t))$, $\dot{V}_{\sss{3}}(t,\xmb(t)) = -W_{\sss{3}}(t,\xmb(t)) \le 0$.
%
Denote then, for convenience
%
\begin{align}	
	\tilde{\umb}(t,\xmb)
	& :=
	\umb(\xmb,T_{\sss{cl}}(t,\bar{\xmb}),\bm{\tau}_{\sss{cl}}(t,\xmb))
	\label{eq:umbtilde}
	\\
	\rQStar(t,\xmb)
	& :=
	\frac{\tilde{\umb}(t,\xmb)}
	{
		\|\tilde{\umb}(t,\xmb)\|
	}
\end{align}
%
where $\umb(\cdot,\cdot,\cdot)$ has been defined in~\eqref{eq:umb}, $\rQStar(t,\xmb)$ is only well defined if $\|\tilde{\umb}(t,\xmb)\| \ne 0$ and where $\rQStar(t,\xmb(t))$ stands for the desired $\rQ(t)$ at time instant $t$.
%

Note that the chosen thrust $T(t)$ can now be rewritten as $T(t) =T_{\sss{Q,cl}}(t,\xmb(t))$, where
%
\begin{align}
	T_{\sss{Q,cl}}(t,\xmb)
	\overset{\sss{\eqref{eq:Thrust},\eqref{eq:umbtilde}}}{=}
	\frac{\nmb\tp\tilde{\umb}(t,\xmb)}{\rQ\tp\nmb}
	\label{eq:ThrustQuadClosedLoop}
\end{align}

Also, denote
%
\begin{align}
	\bm{\epsilon}_{\sss{\theta}}(t,\xmb^{\sss{e}}) 
	&
	:= \emb_{\sss{\theta}}(\xmb^{\sss{e}},T_{\sss{cl}}(t,\bar{\xmb}),\bm{\tau}_{\sss{cl}}(t,\xmb))
	\\
	& =
	\frac{1}{\mQ \Length \rQ\tp\nmb}
	\sk{\nmb } 
	\sk{\rQ}\rQ^{\sss{\star}} \|\tilde{\umb}(t,\xmb)\|,
	\label{eq:ErrorVectorField}
\end{align}
%
and
%
\begin{align}
	\fmb_{\sss{d}}^{\sss{cl}}(t,\xmb^{\sss{e}})
	=
	\fmb_{\sss{u}}^{\sss{cl}}(t,\xmb) 
	+ 
	\begin{bmatrix}
		\zvec_{\sss{9}}
		\\
		\bm{\epsilon}_{\sss{\theta}}(t,\xmb^{\sss{e}})
	\end{bmatrix}
\end{align}
%
where $\fmb_{\sss{d}}^{\sss{cl}}(t,\xmb^{\sss{e}})$ is the vector field $\fmb_{\sss{u}}^{\sss{cl}}(t,\xmb) $ disturbed by the error $\bm{\epsilon}_{\sss{\theta}}(t,\xmb^{\sss{e}})$.
%
Finally, denote
%
\begin{align}	
	\Scale[0.87]{
		\wQStar(t,\xmb^{\sss{e}})
		:=
		\sk{\rQStar(t,\xmb)}
		\frac{
			\frac{\partial \tilde{\umb}(t,\xmb)}{\partial t}
			+
			\frac{\partial \umb\tp(\xmb,T_{\sss{cl}}(t,\bar{\xmb}),\bm{\tau}_{\sss{cl}}(t,\xmb))}{\partial \xmb}
					\fmb_{\sss{d}}^{\sss{cl}}(t,\xmb)
		}
		{
			\|\tilde{\umb}(t,\xmb)\|
		}
	}
	\label{eq:OmegaQuadStar}
\end{align}
%
where $\wQStar(t,\xmb^{\sss{e}})$ is the angular velocity of $\rQStar(t,\xmb)$ for $ \dot{\xmb}(t)  = \fmb_{\sss{d}}^{\sss{cl}}(t,\xmb^{\sss{e}}(t)) $, i.e., $\rQStarDot(t,\xmb(t)) = \sk{\wQStar(t,\xmb^{\sss{e}}(t))} \rQStar(t,\xmb(t))$.

Now, if we choose
%
\begin{align}
	& \TensionStar(t) = T_{\sss{cl}}(t,\bar{\xmb}(t)),
	\\
	& \TauCable(t) = \bm{\tau}_{\sss{cl}}(t,\xmb(t)),
\end{align}
%
it follows that
%
\begin{align}
	 & \frac{\partial V_{\sss{3}}(t,\xmb)}{\partial t}
	+
	\frac{\partial V_{\sss{3}}(t,\xmb)}{\partial \xmb}
	\fmb_{\sss{d}}^{\sss{cl}}(t,\xmb(t))
	\\
	 = &
	 \frac{\partial V_{\sss{3}}(t,\xmb)}{\partial t}
	+
	\frac{\partial V_{\sss{3}}(t,\xmb)}{\partial \xmb}
	(\fmb_{\sss{u}}^{\sss{cl}}(t,\xmb(t)) + [\zvec_{\sss{9}}\tp  \, \bm{\epsilon}_{\sss{\theta}}\tp(t,\xmb^{\sss{e}})]\tp)
	=
	\\
	= &
	-
	W_{\sss{3}}(t,\xmb)
	+
	k_{\sss{\omega}}
	\emb_{\sss{\omega}}\tp(t,\xmb)
	\sk{\nmb} 
	\sk{\nmb}
	\bm{\epsilon}_{\sss{\theta}}(t,\xmb^{\sss{e}})
	\\
	\overset{\sss{\eqref{eq:W3}}}{=} &
	-
	W_{\sss{3}}(t,\xmb)
	-
	k_{\sss{\omega}}
	\emb_{\sss{\omega}}\tp(t,\xmb)
	\bm{\epsilon}_{\sss{\theta}}(t,\xmb^{\sss{e}})	
	\label{eq:W3Altered}
\end{align}

Let us now introduce $\tilde{\xi}(t,\xmb^{\sss{e}}) = 1 - \rQ\tp \rQStar(t,\xmb)$ and 
%
\begin{align}
	V_{\sss{4}}(t,\xmb^{\sss{e}})
	=
	V_{\sss{3}}(t,\xmb)
	+
	\tilde{V}_{\sss{\theta}}(\tilde{\xi}(t,\xmb^{\sss{e}}))
\end{align}
%
for which it follows (for brevity, denote $\tilde{V}'_{\sss{\theta}}(\cdot) =  \tilde{V}'_{\sss{\theta}}(\tilde{\xi}(t,\xmb^{\sss{e}}))$)
%
\begin{align}
	 & \frac{\partial V_{\sss{4}}(t,\xmb)}{\partial t}
	+
	\frac{\partial V_{\sss{4}}(t,\xmb)}{\partial \xmb}
	\begin{bmatrix}
			\fmb_{\sss{d}}^{\sss{cl}}(t,\xmb(t))
			\\
			\sk{\RQ(t)\wQ} \rQ
	\end{bmatrix}
	=
	\\
	&
	\overset{\sss{\eqref{eq:W3Altered},\eqref{eq:OmegaQuadStar}}}{=}
	- W_{\sss{3}}(t,\xmb)
	\\
	&
	-
	k_{\sss{\omega}}
	\emb_{\sss{\omega}}\tp(t,\xmb)
	\bm{\epsilon}_{\sss{\theta}}(t,\xmb^{\sss{e}})		
	+
	\tilde{V}'_{\sss{\theta}}(\cdot)
	(\sk{\rQStar} \rQ)\tp
	\left(
		\RQ(t)\wQ
		-
		\wQStar
	\right)
	\\
	&
	\overset{\sss{\eqref{eq:ErrorVectorField}}}{=}
	- W_{\sss{3}}(t,\xmb)
	+
	\tilde{V}'_{\sss{\theta}}(\tilde{\xi}(t,\xmb^{\sss{e}})) 
	(\sk{\rQStar} \rQ)\tp\cdot
	\\	
	&	
	\cdot
	\bigg(
		\RQ(t)\wQ
		-
		\wQStar(t,\xmb^{\sss{e}})
		+
		\frac{k_{\sss{w}}}{\tilde{V}'_{\sss{\theta}}(\cdot)}
		\frac{1}{\mQ \Length \rQ\tp\nmb}
		\sk{\nmb } 
		\emb_{\sss{\omega}}(t,\xmb)
		\|\tilde{\umb}(t,\xmb)\|				
	\bigg)
	\\
	&
	= :
	- W_{\sss{3}}(t,\xmb)
	+
	\tilde{V}'_{\sss{\theta}}(\tilde{\xi}(t,\xmb^{\sss{e}})) 
	(\sk{\rQStar} \rQ)\tp\cdot
	\\	
	&	
	\cdot
	\bigg(
		\RQ(t)\wQ
		-
		\wQStar(t,\xmb^{\sss{e}})
		-
		\bm{\varepsilon}(t,\xmb^{\sss{e}})
	\bigg)	
	\\
	& :=
	-
	\tilde{W}_{\sss{4}}(t,\xmb^{\sss{e}},\wQ).
	\label{eq:W4Tilde}
\end{align}
%
As such, we if define
%
\begin{align}
	& 
	\bm{\omega}_{\sss{Q,cl}}(t,\xmb^{\sss{e}})
	: =
	\RQ\tp(t)
	\left(
		\wQStar(t,\xmb^{\sss{e}})
		+
		\tilde{k}_{\sss{\theta}}
		\sk{\rQ}
		\rQStar
		+
		\bm{\varepsilon}(t,\xmb^{\sss{e}})			
	\right)
	\\
	& =
	\RQ\tp(t)\wQStar(t,\xmb^{\sss{e}})
	+
	\tilde{k}_{\sss{\theta}}
	\sk{\embThree}
	\RQ\tp(t)
	\rQStar
	+
	\bm{\varepsilon}(t,\xmb^{\sss{e}}),
	\label{eq:OmegaQuadClosedLoop}
\end{align}
%
and choose $\wQ(t) = \bm{\omega}_{\sss{Q,cl}}(t,\xmb^{\sss{e}}(t))$, then 
%
\begin{align}
	&
	\tilde{W}_{\sss{4}}(t,\xmb^{\sss{e}},\bm{\omega}_{\sss{Q,cl}}(t,\xmb^{\sss{e}}))
	\overset{\sss{\eqref{eq:W4Tilde}}}{=}
	-
	W_{\sss{3}}(t,\xmb)
	-
   	\tilde{k}_{\sss{\theta}}
   	\tilde{V}'_{\sss{\theta}}(\cdot) \| \sk{\rQ} \rQStar\|^{2}
   	\\
   	= &
   	-
   	W_{\sss{3}}(t,\xmb)
   	-
   	\tilde{k}_{\sss{\theta}}
   	\tilde{V}'_{\sss{\theta}}(\tilde{\xi}(t,\xmb^{\sss{e}}))
   	\tilde{\xi}(t,\xmb^{\sss{e}}) (2 - \tilde{\xi}(t,\xmb^{\sss{e}}))
   	\\
   	=: &
   	- 
   	W_{\sss{4}}(t,\xmb^{\sss{e}}) \le 0,
\end{align}
%
and for $\dot{\xmb}^{\sss{e}}(t) = \fmb(t,\xmb^{\sss{e}}(t),T_{\sss{cl}}(t,\bar{\xmb}(t)),\bm{\tau}_{\sss{cl}}(t,\xmb(t)),\bm{\omega}_{\sss{Q,cl}}(t,\xmb^{\sss{e}}(t)))$, then $\dot{V}_{\sss{4}}(t,\xmb^{\sss{e}}(t)) = - W_{\sss{4}}(t,\xmb^{\sss{e}}(t)) \le 0$.

Denote $\nmb_{\sss{0}}^{\sss{\star}} = \nmb^{\sss{\star}}(0,\zvec_{\sss{3}},\zvec_{\sss{3}})$, $\xmb^{\sss{0}} = [\zvec_{\sss{6}}\tp \, \nmb_{\sss{0}}^{\sss{\star T}} \, \zvec_{\sss{3}}\tp]\tp $, $\rQStarO = \rQStar(0,\xmb^{\sss{0,T}})$, $\xmb^{\sss{e,0}} = [\xmb^{\sss{0,T}} \, \rQStarOTP]\tp $
%
%\begin{align}
%	\xmb^{\sss{0}} =
%	\begin{bmatrix}
%		\zvec_{\sss{6}}
%		\\
%		\nmb^{\sss{\star}}(0,\zvec_{\sss{3}},\zvec_{\sss{3}})
%		\\
%		\zvec_{\sss{3}}
%	\end{bmatrix}
%	\,
%	,
%	\xmb^{\sss{e,0}} =
%	\begin{bmatrix}
%		\xmb^{\sss{0}}
%		\\
%		\rQStar(0,\xmb^{\sss{0}})
%	\end{bmatrix},
%\end{align}
%
and $\mathcal{N}(r,\xmb^{\sss{e,0}}) = \{ (\pmb,\vmb,\nmb,\emb_{\sss{\omega}},\rQ) \in \Rn[3] \times \Rn[3] \times \mathcal{S}^{\sss{2}} \times \Rn[3] \times \mathcal{S}^{\sss{2}}: \|\pmb\| \le r  \wedge  \|\vmb\| \le r \wedge 1 - \nmb\tp\nmb_{\sss{0}}^{\sss{\star}} \le 2 \frac{r}{1 + r}  \wedge \|\emb_{\sss{\omega}} \| \le r \wedge 1 - \rQ\tp\rQStarO  \le 2 \frac{r}{1 + r} \}$ as a neighborhood around $\xmb^{\sss{e,0}}$.

In order to invoke the results from~\cite{}, $\gmb(t)$ needs to satisfy some constraints:  in particular,
%
\begin{align}
	|\embThree\aLstar(t)| < g \forall t \ge 0,	
\end{align}
%
and $\|\pmb_{\sss{L}}^{\sss{\star(2)}}(\cdot)\|_{\sss{\infty}}, \|\pmb_{\sss{L}}^{\sss{\star(3)}}(\cdot)\|_{\sss{\infty}}, \|\pmb_{\sss{L}}^{\sss{\star(4)}}(\cdot)\|_{\sss{\infty}} <\infty$. 
%
In this problem, we also require $\|\pmb_{\sss{L}}^{\sss{\star(5)}}(\cdot)\|_{\sss{\infty}} <\infty$.
%
Notice that $T_{\sss{cl}}(t,\bar{\xmb})$ in~\eqref{eq:ThrustClosedLoop} is positive if $\nmb\tp \nmb^{\sss{\star}}(t,\pmb,\vmb) > 0$. 
%
If we choose $\epsilon = 1$ and  $\nmb\tp(0) \nmb^{\sss{\star}}(0,\pmb(0),\vmb(0)) > 0$, we can then guarantee that $\nmb\tp(t) \nmb^{\sss{\star}}(t,\pmb(t),\vmb(t)) > 0$ for all $t \ge 0$ (this follows from the fact that $V_{\sss{\theta}}(\xi(t,\bar{\xmb}(t))) \le V_{\sss{4}}(t,\xmb^{\sss{e}}(t)) \le V_{\sss{4}}(0,\xmb^{\sss{e}}(0))$).
%
As such, since $T(t)$ {eq:TensionFinalQuad}
 

\begin{thm}
	Consider the system~\eqref{eq:f1}-\eqref{eq:f3}, with $\bmb = \zvec$.
	%
	If $T(t) = T_{\sss{Q,cl}}(t,\xmb(t))$ as in~\eqref{eq:ThrustQuadClosedLoop}, and $\wQ(t) = \bm{\omega}_{\sss{Q,cl}}(t,\xmb^{\sss{e}}(t))$ as in~\eqref{eq:OmegaQuadClosedLoop}, then there exists $r > 0$ such that if $[\pmb\tp(0) \, \vmb\tp(0) \, \nmb\tp(0) \, \wL\tp(0) \, \rQ\tp(0)]\tp \in \mathcal{N}(r,\xmb^{\sss{e,0}})$ then $\lim_{\sss{t \rightarrow \infty}} \pmb(t) = \zvec$.
\end{thm}

==> SetUps/GenericTerms.tex <==
% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% GLOSSARY
% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %

% create new database
\newcommand\GlossaryName{Glossary}
\newgidx{glossary}{\GlossaryName} 

% default database so I dont have to write \newterm[database=index] every time
\DTLgidxSetDefaultDB{glossary} 

%% EXAMPLE
%\newterm 
% [% 
% % label, sort, parent, text, description, plural, symbol, short, long, shortplural, longplural, see, seealso
%   description={a rectangular table of elements},% brief description 
%   plural={matrices}% the plural 
% ]% 
% {matrix}% the name 
%% OPTIONS
%\gls{matrix}
%\Gls{matrix}
%\glspl{matrix}
%\Glspl{matrix}

% EXAMPLE
\newterm 
 [% 
   description={a rectangular table of elements},% brief description 
   plural={matrices},% the plural 
   symbol = {$\mathcal{\mathcal{R}}$}
 ]% 
 {matrix}% the name 

% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% ACRONYMS
% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% create new database
\newcommand\AcronymsName{Acronyms}
\newgidx{acronym}{\AcronymsName} 

% default database so I dont have to write \newterm[database=index] every time
\DTLgidxSetDefaultDB{acronym} 

\newacro{svm}{support vector machine} 


% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% NOTATION
% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% create new database 
\newcommand\NotationName{Notation}
\newgidx{notation}{\NotationName} 

% default database so I dont have to write \newterm[database=index] every time
\DTLgidxSetDefaultDB{notation} 
      

%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={ContinuousFunction}, % label 
	description={Function whose $i^{\text{th}}$ derivative is continuous.},% 
	sort={ContinuousFunction}% 
]% 
{$\Cont{i}$}
\newcommand{\Cont}[1]{\mathcal{C}^{(#1)}}



\newterm 
[% 
	label={SO3}, % label 
	description={Space of rotation matrices in $\mathbb{R}^{3 \times 3}$.},% 
	sort={SpecialOrthogonalGroup}% 
]% 
{$\SO$}
\newcommand{\SO}[1][3]{\mathcal{SO}(#1)}

%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={R}, % label 
	description={$\RFL \coloneqq \Rmat \in \gls{SO3}$ is the Leader-Follower formation rotation matrix.},% 
	sort={r}% 
]% 
{$\RFL \coloneqq \Rmat$}
\newcommand{\RFL}{\RmatAB{F}{L}}
\newcommand{\RFLDot}{\RdmatAB{F}{L}}
\newcommand{\RDot}{\dot{\Rmat}}

\newterm 
[% 
	label={r1}, % label 
	parent ={R},
	description={First column of matrix $\RFL$.},% 
	sort={ra}% 
]% 
{$\rmb_{1}$}
\newcommand{\rOne}{\rmb_{1}}
\newcommand{\rOneDot}{\dot{\rmb}_{1}}


\newterm 
[% 
	label={r2}, % label 
	parent ={R},
	description={Second column of matrix $\RFL$.},% 
	sort={rb}% 
]% 
{$\rTwo$}
\newcommand{\rTwo}{\rmb_{2}}

\newterm 
[% 
	label={r3}, % label 
		parent ={R},
	description={Third column of matrix $\RFL$.},% 
	sort={rc}% 
]% 
{$\rThree$}
\newcommand{\rThree}{\rmb_{3}}
\newcommand{\rThreeStar}{\rmb_{3}^{\star}}

\newcommand{\rThreeTR}{\rmb_{3}^{\sss{tr}}}


\newterm 
[% 
	label={r11}, % label 
	parent = {R},
	description={First element of \gls{r1}.},% 
	sort={raa}% 
]% 
{$\rOneOne$}
\newcommand{\rOneOne}{\text{r}_{11}}
\newcommand{\rOneOneDot}{\dot{\text{r}}_{11}}

\newterm 
[% 
	label={r12}, % label 
	parent = {R},
	description={Second element of \gls{r1}.},% 
	sort={rab}% 
]% 
{$\rOneTwo$}
\newcommand{\rOneTwo}{\text{r}_{12}}
\newcommand{\rOneTwoDot}{\dot{\text{r}}_{12}}

\newterm 
[% 
	label={r13}, % label 
	parent = {R},
	description={Third element of \gls{r1}.},% 
	sort={rac}% 
]% 
{$\rOneThree$}
\newcommand{\rOneThree}{\text{r}_{13}}

\newcommand{\rTwoOne}{\text{r}_{21}}
%\newcommand{\rTwoOneStar}{\text{r}_{21}^{\star}}
\newcommand{\rTwoTwo}{\text{r}_{22}}
\newcommand{\rTwoTwoStar}[1][]{\text{r}_{22}^{\star{#1}}}
\newcommand{\rTwoThree}{\text{r}_{23}}
\newcommand{\rTwoThreeStar}[1][]{\text{r}_{23}^{\star{#1}}}

\newcommand{\rThreeOne}{\text{r}_{31}}
\newcommand{\rThreeOneDot}{\dot{\text{r}}_{31}}
\newcommand{\rThreeOneStar}[1][]{\text{r}_{31}^{\star{#1}}}
\newcommand{\rThreeTwo}{\text{r}_{32}}
\newcommand{\rThreeTwoStar}[1][]{\text{r}_{32}^{\star{#1}}}
\newcommand{\rThreeThree}{\text{r}_{33}}
\newcommand{\rThreeThreeStar}[1][]{\text{r}_{33}^{\star{#1}}}

\newcommand{\rThreeOneTR}[1][]{\text{r}_{31}^{\sss{tr}{#1}}}
\newcommand{\rThreeThreeTR}[1][]{\text{r}_{33}^{\sss{tr}{#1}}}

%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={deltar1}, % label 
	description={Difference between solution $\rOne$ and equilibrium solution $\rOneStar$, i.e. $\DeltarOne = \rOne -\rOneStar$.},% 
	sort={deltaA}% 
]% 
{$\DeltarOne$}
\newcommand{\DeltarOne}{\delta \rOne}
\newcommand{\DeltarOneDot}{\delta \rOneDot}

\newterm 
[% 
	label={deltar2}, % label 
	description={Virtual displacement around nominal motion $\rOneStar(t)$.},% 
	sort={deltaB}% 
]% 
{$\DeltarOneV$}
\newcommand{\DeltarOneV}{\delta \rOne^{v}}
\newcommand{\DeltarOneVTP}{\delta \rOne^{v \sss{T}}}
\newcommand{\DeltarOneVDot}{\delta \rOneDot^{v}}

%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={Rstar}, % label 
	description={$\Rmat^{\star}\in \gls{SO3}$ is the equilibrium Leader-Follower formation matrix.},% 
	sort={rstar}% 
]% 
{$\Rstar$}
\newcommand{\Rstar}{\Rmat^{\star}}
\newcommand{\RstarTP}{\Rmat^{\star \sss{T}}}
\newcommand{\RstarDot}{\dot{\Rmat}^{\star}}
\newcommand{\RstarOne}{\Rmat_1^{\star}}
\newcommand{\RstarTwo}{\Rmat_2^{\star}}

\newcommand{\RTR}{\Rmat^{\sss{tr}}}
\newcommand{\RNonTR}{\Rmat^{\sss{n-tr}}}

\newterm 
[% 
	label={r1star}, % label 
	parent = {Rstar},
	description={First column of matrix \gls{Rstar}.},% 
	sort={rastar}% 
]% 
{$\rOneStar$}
\newcommand{\rOneStar}{\rmb_{1}^{\star}}
\newcommand{\rOneStarNot}{\bar{\rmb}_{1}^{\star}}
\newcommand{\rOneStarTP}{\rmb_{1}^{\star \sss{T} }}
\newcommand{\rOneStarDot}{\dot{\rmb}_{1}^{\star}}

\newcommand{\rOneTR}{\rmb_{1}^{\sss{tr}}}
\newcommand{\rOneTRTP}{\rmb_{1}^{\sss{tr}\, \sss{T}}}
\newcommand{\rOneTRDot}{\dot{\rmb}_{1}^{\sss{tr}}}
\newcommand{\rOneTRNot}{\bar{\rmb}_{1}^{\sss{tr}}}

\newcommand{\rOneNonTR}{\rmb_{1}^{\sss{n-tr}}}
\newcommand{\rOneNonTRTP}{\rmb_{1}^{\sss{n-tr} \, \sss{T}}}
\newcommand{\rOneNonTRNot}{\bar{\rmb}_{1}^{\sss{n-tr}}}

\newterm 
[% 
	label={r11Star}, % label 
	parent = {Rstar},
	description={First element of $\rOneStar$.},% 
	sort={rastara}% 
]% 
{$\rOneOneStar$}
\newcommand{\rOneOneStar}[1][{}]{\text{r}_{11}^{\star{#1}}}
\newcommand{\rOneOneStarDot}{\dot{\text{r}}_{11}^{\star}}

\newcommand{\rOneOneTR}[1][{}]{\text{r}_{11}^{\sss{tr}{#1}}}
\newcommand{\rOneOneTRNot}[1][{}]{\bar{\text{r}}_{11}^{\sss{tr}{#1}}}

\newterm 
[% 
	label={r12Star}, % label 
	parent = {Rstar},
	description={Second element of $\rOneStar$.},% 
	sort={rastarb}% 
]% 
{$\rOneTwoStar$}
\newcommand{\rOneTwoStar}[1][]{\text{r}_{12}^{\star{#1}}}

\newterm 
[% 
	label={r13Star}, % label 
	parent = {Rstar},
	description={Third element of $\rOneStar$.},% 
	sort={rastarc}% 
]% 
{$\rOneThreeStar$}
\newcommand{\rOneThreeStar}[1][]{\text{r}_{13}^{\star{#1}}}

\newterm 
[% 
	label={r2star}, % label 
	parent = {Rstar},
	description={Second column of matrix \gls{Rstar}.},% 
	sort={rbstar}% 
]% 
{$\rTwoStar$}
\newcommand{\rTwoStar}{\rmb_{2}^{\star}}

\newterm 
[% 
	label={r21Star}, % label 
	parent = {Rstar},
	description={First element of $\rTwoStar$.},% 
	sort={rbstara}% 
]% 
{$\rTwoOneStar$}
\newcommand{\rTwoOneStar}[1][]{\text{r}_{21}^{\star{#1}}}

\newcommand{\rTwoOneTR}[1][]{\text{r}_{21}^{\sss{tr}{#1}}}
\newcommand{\rTwoOneNonTR}[1][]{\text{r}_{21}^{\sss{n-tr}{#1}}}

\newterm 
[% 
	label={r3star}, % label 
	parent = {Rstar},
	description={Third column of matrix \gls{Rstar}.},% 
	sort={rcstar}% 
]% 
{\ensuremath{\rmb_{3}^{\star}}}


%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={dCM}, % label 
	description={Distance vector between \emph{virtual} Follower center of mass and Leader, specified in \emph{virtual} Follower reference frame.},% 
	sort={d}% 
]% 
{$\dCM$}
\newcommand{\dCM}{\dmb^{\sss{CM}}}

\newterm 
[% 
	label={d}, % label 
	description={Distance vector between \emph{virtual} Follower and Leader, specified in \emph{virtual} Follower reference frame.},% 
	sort={d}% 
]% 
{\ensuremath{\dmb}}

\newcommand{\dI}{ {}^{\sss{\mathcal{I}}}\dmb}

\newterm 
[% 
	label={dx}, % label 
	parent = {d},
	description={Longitudinal component of vector \gls{d}.},% 
	sort={da}% 
]% 
{$\dx$}
\newcommand{\dx}{\text{d}_{\text{x}}}

\newterm 
[% 
	label={dy}, % label 
	parent = {d},
	description={Lateral component of vector \gls{d}.},% 
	sort={db}% 
]% 
{$\dy$}
\newcommand{\dy}{\text{d}_{\text{y}}}

\newterm 
[% 
	label={dz}, % label 
	parent = {d},
	description={Vertical component of vector \gls{d}.},% 
	sort={dc}% 
]% 
{$\dz$}
\newcommand{\dz}{\text{d}_{\text{z}}}

\newterm 
[% 
	label={dzy}, % label 
	parent = {d},
	description={Norm of lateral and vertical components of vector \gls{d}, i.e. $\dyz = \sqrt{\dy^2+\dz^{2}}$.},% 
	sort={dd}% 
]% 
{$\dyz$}
\newcommand{\dyz}{\text{d}_{\text{yz}}}

\newterm 
[% 
	label={lambdazy}, % label 
	parent = {d},
	description={$\ldyz= \left(\frac{\dyz}{\dx}\right)^2$.},% 
	sort={ddB}% 
]% 
{$\ldyz$}
\newcommand{\ldyz}{\lambda_{\text{yz}}}

%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={DirectionLong}, % label 
	description={Longitudinal direction},% 
	sort={DirectionsBasisA}% 
]% 
{$\nLong$}
\newcommand{\nLong}{\nmb_{\sss{long}}}

\newterm 
[% 
	label={DirectionLat}, % label 
	description={Lateral direction},% 
	sort={DirectionsBasisB}% 
]% 
{$\nLat$}
\newcommand{\nLat}{\nmb_{\sss{lat}}}

\newterm 
[% 
	label={DirectionVert}, % label 
	description={Vertical direction},% 
	sort={DirectionsBasis}% 
]% 
{$\nV$}
\newcommand{\nV}{\nmb_{\sss{v}}}

\newcommand{\dLong}{\text{d}_{\sss{long}}}
\newcommand{\dLongDot}{\dot{\text{d}}_{\sss{long}}}
\newcommand{\dLat}{\text{d}_{\sss{lat}}}

\newcommand{\dRB}{\dmb^{\sss{RB}}}

%---------------------------------------------------------- %
%---------------------------------------------------------- %
\newterm 
[% 
	label={CanonicalBasis}, % label 
	description={Inertial Reference Frame.},% 
	sort={CanonicalBasis}% 
]% 
{\fr{I}}

\newterm 
[% 
	label={e1}, % label
	parent = {CanonicalBasis}, 
	description={ $\emb_1 \in \UnitSet$ is the first vector of the canonical basis in $\mathbb{R}^{3}$.},% 
	sort={CanonicalBasisA}% 
]% 
{$\eOne$}
\newcommand{\eOne}{\emb_1}

\newterm 
[% 
	label={e2}, % label
	parent = {CanonicalBasis}, 
	description={ $\emb_2 \in \UnitSet$ is the second vector of the canonical basis in $\mathbb{R}^{3}$.},% 
	sort={CanonicalBasisB}% 
]% 
{$\eTwo$}
\newcommand{\eTwo}{\emb_2}

\newterm 
[% 
	label={e3}, % label
	parent = {CanonicalBasis}, 
	description={ $\emb_3 \in \UnitSet$ is the third vector of the canonical basis in $\mathbb{R}^{3}$.},% 
	sort={CanonicalBasisC}% 
]% 
{$\eThree$}
\newcommand{\eThree}{\emb_3}


%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={Follower}, % label 
	description={Follower's Reference Frame.},% 
	sort={FollowerFrame}% 
]% 
{\fr{F}}

\newterm 
[% 
	label={RF}, % label 
	parent = {Follower},
	description={Rotation matrix associated to \fr{F}.},% 
	sort={FollowerRotationMatrix}% 
]% 
{$\RF$}
\newcommand{\RF}{\RmatAB{F}{I}}
\newcommand{\RFStar}{\RmatAB{F}{I}^{\star}}
\newcommand{\RFTP}{\RmatAB{I}{F}}
\newcommand{\RFDot}{\RdmatAB{F}{I}}

\newcommand{\RFtr}{\Rmat_{\sss{\mathcal{F}}}^{\sss{tr}}}
\newcommand{\RFnontr}{\bar{\Rmat}_{\sss{\mathcal{F}}}^{\sss{n-tr}}}

\newterm 
[% 
	label={pF}, % label 
	parent = {Follower},
	description={Follower's position in \fr{I}.},% 
	sort={AAPositionFollowerA}% 
]% 
{$\pF$}
\newcommand{\pF}[1][{}]{\pmb_{\sss{\mathcal{F}_{#1}}}}
\newcommand{\pFDot}{\dot{\pmb}_{\sss{\mathcal{F}}}}

\newterm 
[% 
	label={pFCM}, % label 
	parent = {Follower},
	description={Follower's center of mass position in \fr{I}.},% 
	sort={AAPositionFollowerB}% 
]% 
{$\pFCM$}
\newcommand{\pFCM}{\ptframe{\pmb}{}{F}^{\sss{CM}}}
\newcommand{\pFCMDot}{\ptframe{\dot{\pmb}}{}{F}^{\sss{CM}}}
\newcommand{\pFtr}{\ptframe{\pmb}{}{F}^{\sss{tr}}}
\newcommand{\pFnontr}{\ptframe{\pmb}{}{F}^{\sss{n-tr}}}
\newcommand{\pFtrNot}{\ptframe{\bar{\pmb}}{}{F}^{\sss{tr}}}

\newterm 
[% 
	label={vF}, % label 
	parent = {Follower},
	description={Follower's velocity in \fr{I}.},% 
	sort={ABVelocityFollowerA}% 
]% 
{$\vF$}
\newcommand{\vF}{\ptframe{\vmb}{}{F}}

\newterm 
[% 
	label={uFComplete}, % label 
	parent = {Follower},
	description={Follower's velocity in \fr{F} (body framed velocity, i.e. $\vF \coloneqq \RF \vFBody$).},% 
	sort={ABVelocityFollowerB}% 
]% 
{$\vFBody$}
\newcommand{\vFBody}{\ptframe{\umb}{}{F}}

\newterm 
[% 
	label={uF}, % label 
	parent = {Follower},
	description={First Component of $\vFBody$, i.e. $\uF = \eOne\tp \vFBody$.},% 
	sort={ABVelocityFollowerBA}% 
]% 
{$\uF$}
\newcommand{\uF}{u_{\sss{F}}}

\newterm 
[% 
	label={vvF}, % label 
	parent = {Follower},
	description={Second Component of $\vFBody$, i.e. $\vvF = \eTwo\tp \vFBody$.},% 
	sort={ABVelocityFollowerBB}% 
]% 
{$\vvF$}
\newcommand{\vvF}{v_{\sss{F}}}

\newterm 
[% 
	label={wF}, % label 
	parent = {Follower},
	description={Third Component of $\vFBody$, i.e. $\wF = \eThree\tp \vFBody$.},% 
	sort={ABVelocityFollowerBC}% 
]% 
{$\wF$}
\newcommand{\wF}{w_{\sss{F}}}

\newterm 
[% 
	label={oF}, % label 
	parent = {Follower},
	description={Follower's reference frame angular velocity specified in \fr{F}.},% 
	sort={ACAngularVelocityFollower}% 
]% 
{$\oF$}
\newcommand{\oF}{\ptframe{\bm{\omega}}{}{F}}

\newterm 
[% 
	label={FollowerCurvature}, % label 
	parent = {Follower},
	description={Follower's path curvature.},% 
	sort={FollowerACurvature}% 
]% 
{$\kF$}
\newcommand{\kF}{\kappa_{\sss{\mathcal{F}}}}

\newterm 
[% 
	label={FollowerTorsion}, % label 
	parent = {Follower},
	description={Follower's path torsion.},% 
	sort={FollowerATorsion}% 
]% 
{$\tF$}
\newcommand{\tF}{\tau_{\sss{\mathcal{F}}}}

\newterm 
[% 
	label={oFp}, % label 
	parent = {Follower},
	description={Roll rate, i.e. $p = \eOne\tp \oF$.},% 
	sort={ACAngularVelocityFollowerA}% 
]% 
{$\roll$}
\newcommand{\roll}{p_{\sss{\mathcal{F}}}}

\newterm 
[% 
	label={oFq}, % label 
	parent = {Follower},
	description={Pitch rate, i.e. $q = \eTwo\tp \oF$.},% 
	sort={ACAngularVelocityFollowerB}% 
]% 
{$\pitch$}
\newcommand{\pitch}{q_{\sss{\mathcal{F}}}}

\newterm 
[% 
	label={oFr}, % label 
	parent = {Follower},
	description={Yaw rate, i.e. $r = \eThree\tp \oF$.},% 
	sort={ACAngularVelocityFollowerC}% 
]% 
{$\yaw$}
\newcommand{\yaw}{r_{\sss{\mathcal{F}}}}


%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={gkL}, % label 
	description={Non-dimensionalized Curvature Parameter, i.e. $\gkL = \kL\dx$},% 
	sort={NoDimensionsCurvatureTorsionA}% 
]% 
{$\gkL$}
\newcommand{\gkL}{\gamma_{\kappa}}
\newcommand{\gkLDot}{\dot{\gamma}_{\kappa}}

\newterm 
[% 
	label={gtL}, % label 
	description={Non-dimensionalized Torsion Parameter, i.e. $\gtL = \tL\dx$},% 
	sort={NoDimensionsCurvatureTorsionB}%
]% 
{$\gtL$}
\newcommand{\gtL}{\gamma_{\tau}}
\newcommand{\gtLDot}{\dot{\gamma}_{\tau}}

\newterm 
[% 
	label={gKL}, % label 
	description={Non-dimensionalized Curvature and Torsion Parameter, i.e. $\gKL = \threerow{\gtL}{0}{\gkL}$},% 
	sort={NoDimensionsCurvatureTorsionC}% 
]% 
{$\gKL$}
\newcommand{\gKL}{\bm{\gamma}_{\bm{\kappa}}}
\newcommand{\gKLDot}{\dot{\bm{\gamma}}_{\bm{\kappa}}}

%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={Leader}, % label 
	description={Leader Frenet Reference Frame.},% 
	sort={LeaderFrame}% 
]% 
{\fr{L}}

\newterm 
[% 
	label={RL}, % label 
	parent = {Leader},
	description={Frenet rotation matrix associated to \fr{I}.},% 
	sort={LeaderRotationMatrix}% 
]% 
{$\RL$}
\newcommand{\RL}{\RmatAB{L}{I}}
\newcommand{\RLTP}{\RmatAB{I}{L}}
\newcommand{\RLDot}{\RdmatAB{L}{I}}

\newterm 
[% 
	label={gL}, % label 
	parent = {Leader},
	description={Parametrization of Leader's path that guarantees unit velocity, i.e. $\Norm{\frac{d \pL(\gL)}{d \gL}} =1$ and $\frac{d \gL(t)}{dt}= \Norm{\vL(t)}$.},% 
	sort={LeaderParametrization}% 
]% 
{\ensuremath{\gamma_{\sss{\mathcal{L}}} }}
\newcommand{\gL}{\ensuremath{\gamma_{\sss{\mathcal{L}}} }}

\newterm 
[% 
	label={fgL}, % label 
	parent = {Leader},
	description={Map between $\gL$ parametrization and the time parametrization.},% 
	sort={LeaderParametrizationMap}% 
]% 
{\ensuremath{f_\gamma}}
\newcommand{\fL}{f_\gamma}

\newterm 
[% 
	label={TL}, % label 
	parent = {Leader},
	description={Leader's path Tangent, i.e. $\TL(\gL)=\frac{d \pL(\gL)}{d \gL}$ or $\TL(t)=\frac{\vL(t)}{\Norm{\vL(t)}}$.},% 
	sort={LeaderPathA}% 
]% 
{$\TL$}
\newcommand{\TL}{\Tmb_{\sss{\mathcal{L}}}}
\newcommand{\TLDot}{\dot{\Tmb}_{\sss{\mathcal{L}}}}

\newterm 
[% 
	label={NL}, % label 
	parent = {Leader},
	description={Leader's path Normal.},% 
	sort={LeaderPathB}% 
]% 
{$\NL$}
\newcommand{\NL}{\Nmb_{\sss{\mathcal{L}}}}

\newterm 
[% 
	label={BL}, % label 
	parent = {Leader},
	description={Leader's path Binormal.},% 
	sort={LeaderPathC}% 
]% 
{$\BL$}
\newcommand{\BL}{\Bmb_{\sss{\mathcal{L}}}}

\newterm 
[% 
	label={KL}, % label 
	parent = {Leader},
	description={$\bm{\kappa}_{\sss{\mathcal{L}}} \in \mathbb{R}^{3}$ such that $\bm{\kappa}_{\sss{\mathcal{L}}} = \tL \eOne  + \kL \eThree$.},% 
	sort={LeaderZGeneralizedCurvature}% 
]% 
{$\KL$}
\newcommand{\KL}{\bm{\kappa}_{\sss{\mathcal{L}}}}
\newcommand{\KLDot}{\dot{\bm{\kappa}}_{\sss{\mathcal{L}}}}

\newterm 
[% 
	label={kL}, % label 
	parent = {Leader},
	description={Leader path curvature.},% 
	sort={LeaderCurvature}% 
]% 
{$\kL$}
\newcommand{\kL}{\kappa_{\sss{\mathcal{L}}}}
\newcommand{\kLmax}{\kappa_{{\sss{\mathcal{L}}}_{\max}}}
\newcommand{\kLmin}{\kappa_{{\sss{\mathcal{L}}}_{\min}}}
\newcommand{\kLDot}{\dot{\kappa}_{\sss{\mathcal{L}}}}


\newterm 
[% 
	label={tL}, % label
	parent = {Leader}, 
	description={Leader path torsion.},% 
	sort={LeaderTorsion}% 
]% 
{$\tL$}
\newcommand{\tL}{\tau_{\sss{\mathcal{L}}}}
\newcommand{\tLDot}{\dot{\tau}_{\sss{\mathcal{L}}}}

\newterm 
[% 
	label={pL}, % label 
	parent = {Leader},
	description={Leader's position in \fr{I}.},% 
	sort={AAPositionLeader}% 
]% 
{$\pL$}
\newcommand{\pL}{\ptframe{\pmb}{}{L}}
\newcommand{\pLDot}{\ptframe{\dot{\pmb}}{}{L}}

\newterm 
[% 
	label={vL}, % label 
	parent = {Leader},
	description={Leader's velocity in \fr{I}.},% 
	sort={ABVelocityLeader}% 
]% 
{$\vL$}
\newcommand{\vL}{\ptframe{\vmb}{}{L}}
\newcommand{\vLDot}{\dot{\vmb}_{\sss{\mathcal{L}}}}

\newterm 
[% 
	label={vLminimum}, % label 
	parent = {Leader},
	description={Minimum Leader's velocity norm, i.e. $\vLmin = \min \Norm{\vL} $},% 
	sort={AEVelocityLeader}% 
]% 
{$\vLmin$}
\newcommand{\vLmin}{v_{\sss{\mathcal{L}}}^{\sss{\min}}}

\newterm 
[% 
	label={aL}, % label 
	parent = {Leader},
	description={Leader's acceleration in \fr{I}.},% 
	sort={ACAccelerationLeader}% 
]% 
{$\aL$}
\newcommand{\aL}{\ptframe{\amb}{}{L}}

\newterm 
[% 
	label={jL}, % label 
	parent = {Leader},
	description={Leader's jerk in \fr{I}.},% 
	sort={ADJerkLeader}% 
]% 
{$\jL$}
\newcommand{\jL}{\ptframe{\jmb}{}{L}}

\newterm 
[% 
	label={oL}, % label 
	parent = {Leader},
	description={Leader's reference frame angular velocity specified in \fr{L}, $\oL \equiv \Norm{\vL} \KL$.},% 
	sort={AEAngularVelocityLeader}% 
]% 
{$\oL$}
\newcommand{\oL}{\ptframe{\bm{\omega}}{}{L}}

%---------------------------------------------------------- %
%---------------------------------------------------------- %


%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={OrderMagnitude}, % label 
	description={Order of Magnitude w.r.t. $n$.},% 
	sort={OrderMagnitude}% 
]% 
{\ensuremath{\mathcal{O}(n)}}
\newcommand{\OM}[1]{\mathcal{O}\left(#1\right)}

%---------------------------------------------------------- %
%---------------------------------------------------------- %


\newterm 
[% 
	label={OFL}, % label 
	description={Angular veclocity of \fr{F} w.r.t. \fr{L} specified in \fr{L}.},% 
	sort={FLOmega}% 
]% 
{$\OFL$}
\newcommand{\OFL}{\ptframe{\bm{\omega}}{L}{F|L}}
\newcommand{\OFLstar}{{}^{\sss{\mathcal{L}}} {\bm{\omega}}_{\sss{\mathcal{F|L}}}^{\star}}

\newterm 
[% 
	label={pFL}, % label 
	description={Position of Follower with respect to \fr{L} specified in \fr{L}.},% 
	sort={FLPositionA}% 
]% 
{$\pFL$}
\newcommand{\pFL}{\ptframe{\pmb}{L}{F|L}}
\newcommand{\pFLStar}{{}^{\sss{\mathcal{L}}}\pmb_{\sss{\mathcal{F|L}}}^{\star}}
\newcommand{\pLFi}[1]{{}^{\mathcal{F}_{#1}}\pmb_{\mathcal{F}_{#1}|\mathcal{L}}}

\newcommand{\pLFL}{\ptframe{\pmb}{L}{L|F}}
\newcommand{\pLFTR}{\ptframe{\pmb}{L}{L|F}^{\sss{tr}}}
\newcommand{\pFLTR}{{}^{\sss{\mathcal{L}}}\pmb_{\sss{\mathcal{F|L}}}^{\sss{tr}}}
\newcommand{\pFLF}{\ptframe{\pmb}{F}{F|L}}
\newcommand{\pFLFCM}{\ptframe{\pmb}{F}{F|L}^{\sss{CM}}}

\newterm 
[% 
	label={pFL2}, % label 
	description={Position of Leader with respect to \fr{F} specified in \fr{F}.},% 
	sort={FLPositionB}% 
]% 
{$\pLF$}
\newcommand{\pLF}{\ptframe{\pmb}{F}{L|F}}


\newterm 
[% 
	label={rOneProj}, % label 
	description={Projection of $\rOne$ over $\rOneStar$, i.e. $\alpha= \rOne\tp \rOneStar$.},% 
	sort={rOneProj}% 
]% 
{\ensuremath{\alpha}}
\newcommand{\rOneProj}{\alpha}
\newcommand{\rOneProjDot}{\dot{\alpha}}

\newterm 
[% 
	label={rOneProj2}, % label 
	description={Defined as 1-$\rOneProj$.},% 
	sort={rOneProjB}% 
]% 
{$\rOneProjB$}
\newcommand{\rOneProjB}{\beta}
\newcommand{\rOneProjBDot}{\dot{\beta}}

\newterm 
[% 
	label={RProj}, % label 
	description={\emph{Projection} of $\Rmat$ over $\Rstar$, i.e. $\Rerror= \Rmat\tp \Rstar$.},% 
	sort={rOneProjC}% 
]% 
{$\Rerror$}
\newcommand{\Rerror}{\Rmat_{\text{e}}}
\newcommand{\RerrorDot}{\dot{\Rmat}_{\text{e}}}


% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %

\newterm 
[% 
	label={Rx}, % label 
	description={Rotation matrix around the first axis.},% 
	sort={rx}% 
]% 
{$\Rx$}
\newcommand{\Rx}{\Rmat_{x}}

\newterm 
[% 
	label={Ry}, % label 
	description={Rotation matrix around the second axis.},% 
	sort={ry}% 
]% 
{$\Ry$}
\newcommand{\Ry}{\Rmat_{y}}

\newterm 
[% 
	label={Rz}, % label 
	description={Rotation matrix around the third axis.},% 
	sort={rz}% 
]% 
{$\Rz$}
\newcommand{\Rz}{\Rmat_{z}}

%---------------------------------------------------------- %
%---------------------------------------------------------- %

\newterm 
[% 
	label={Sstar}, % label 
	description={},% 
	sort={Sstar}% 
]% 
{$\Sstar$}
\newcommand{\Sstar}[1][0]{\text{s}^{\star\sss{(#1)}}}
\newcommand{\SStar}{\textbf{s}^{\star}}
\newcommand{\SStarDot}{\dot{\textbf{s}}^{\star}}
\newcommand{\ASStar}{\mat{A}_{\SStar}}
\newcommand{\PSStar}{\mat{P}_{\SStar}}
\newcommand{\QSStar}{\mat{Q}_{\SStar}}

%---------------------------------------------------------- %
%---------------------------------------------------------- %

% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% INDEX
% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% create new database
\newcommand\IndexName{Index}
\newgidx{index}{\IndexName}

% default database so I dont have to write \newterm[database=index] every time
\DTLgidxSetDefaultDB{index} 


% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% FUNCTIONS
% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% create new database 
\newcommand\FunctionName{Functions}
\newgidx{functions}{\FunctionName} 

% default database so I dont have to write \newterm[database=index] every time
\DTLgidxSetDefaultDB{functions} 

\newterm 
[% 
	label={Skew}, % label 
	description={The map $\text{S}(\xmb): \mathbb{R}^{3}\rightarrow\mathbb{R}^{3\times 3}$ yields a cross product skew symmetric matrix such that $\text{S}(\amb)\bmb = \amb \times \bmb$},% 
	sort={Skew}% 
]% 
{$\Skew{}$}
\newcommand{\Skew}[1]{\mathcal{S}\left(#1\right)}

\newterm 
[% 
	label={UnSkew}, % label 
	description={The map $\UnSkew{\Amb}: AS \rightarrow\mathbb{R}^{3}$ yields the vector that produces the skew symmetric matrix $\Amb$ such that $\text{S}(\UnSkew{\Amb}) = \Amb$, where $AS$ is the space of the anti-symmetric matrices, i.e. $AS=\{\Amb \in \mathbb{R}^{3\times 3}: \Amb=-\Amb\tp\}$},% 
	sort={SkewB}% 
]% 
{$\UnSkew{}$}
\newcommand{\UnSkew}[1]{\text{S}^{-1}\left(#1\right)}

\newterm 
[% 
	label={Norm}, % label 
	description={The map $\|\xmb\|: \mathbb{R}^{n}\rightarrow\mathbb{R}$ yields the norm of vector $\xmb$ such that $\|\xmb\| = \sqrt{\xmb\tp \xmb}$},% 
	sort={Norm}% 
]% 
{\ensuremath{\|\xmb\|}}
\newcommand{\Norm}[1]{\ensuremath{\left\| #1 \right\|}}

\newterm 
[% 
	label={OrthogonalProjection}, % label 
	description={The map $\Pi(\xmb):\mathbb{R}^{3}\backslash \{\textbf{0}\} \rightarrow \mathbb{R}^{3\times 3}$, where $\Pi(\xmb)=-\text{S}\left(\frac{\xmb}{\Norm{\xmb}}\right)^2$ yields a matrix that represents the orthogonal projection operator onto the subspace perpendicular to $\xmb$.},% 
%	description={The map $\Pi(\xmb):\mathbb{R}^{3} \rightarrow \mathbb{R}^{3\times 3}$, where $\Pi(\xmb)=−\Skew{\frac{\xmb}{\Norm{\xmb}}}^2$ yields a matrix that represents the orthogonal projection operator onto the subspace perpendicular to $\xmb$.},% 
	sort={OrthogonalProjection}% 
]% 
{$\OP{\xmb}$}
\newcommand{\OP}[1]{\Pi\left( #1 \right)}


% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% SETS
% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %
% create new database 
\newcommand\SetsName{Sets}
\newgidx{sets}{\SetsName} 

% default database so I dont have to write \newterm[database=index] every time
\DTLgidxSetDefaultDB{sets} 

\newterm 
[% 
	label={SO}, % label 
	description={Space of rotation matrices in $\mathbb{R}^{n\times n}$, i.e. \\ 
	$\text{SO}(n)~=
	~\left\{
		\Rmat \in \mathbb{R}^{n\times n}:
		\Rmat\tp \Rmat = \Idmat, \det \Rmat = +1 
	\right\}$
	\\},% 
	sort={SpecialOrthogonalGroup}% 
]% 
{\ensuremath{\text{SO}(n)}}

\newterm 
[% 
	label={UnitVector}, % label 
	description={Set of all unit vectors in $\mathbb{R}^{3}$, i.e. $\UnitSet = \{\xmb \in \mathbb{R}^{3} : \Norm{\xmb}=1\}$\\},% 
	sort={SetUnitVectors}% 
]% 
{$\UnitSet$}
\newcommand{\UnitSet}{\Omega_\text{N}}

% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %

\newterm 
[% 
	label={UnitVectorPositiveComponentEpsilon}, % label 
	description={Set of all unit vectors in $\mathbb{R}^{3}$ with limited longitudinal component, i.e. \\ 
	$
		\Omega_\text{N}^{\star}(\epsilon) = 
		\{
			\xmb \in \mathbb{R}^{3} :
			\Norm{\xmb}=1
			\wedge 
			\xmb\tp \eOne \sign{\dx} >\epsilon^2 ,
			\epsilon \in \SetOne
		\}
	$\\},% 
	sort={SetUnitVectorsPositiveComponentA}% 
]% 
{$\ONstarEpsilon$}
\newcommand{\ONstarEpsilon}[1][\epsilon]{\Omega_\text{1}(#1)}
\newcommand{\ONstarEpsilonStar}{\Omega_\text{1}^{\star}(\epsilon)}

\newterm 
[% 
	label={UnitVectorPositiveComponent}, % label 
	description={Set of all unit vectors in $\mathbb{R}^{3}$ with longitudinal component signed as $\dx$, i.e. \\
		$
			\Omega_\text{N}^{\star} =
			\{
				\xmb \in \mathbb{R}^{3} :
				\Norm{\xmb}=1 
				\wedge
				\xmb\tp \eOne \sign{\dx} >0 
			\}
			\equiv
			\Omega_\text{N}^{\star}(0)
		$\\},% 
	sort={SetUnitVectorsPositiveComponentB},%
	parent={UnitVectorPositiveComponentEpsilon}
]% 
{\ensuremath{\Omega_\text{N}^{\star}}}
\newcommand{\ONstar}{\Omega_\text{N}^{\star}}

% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %

\newterm 
[% 
	label={TimeSet}, % label 
	description={Time Domain, i.e. $\Omega_{\sss{t_0}} = \{t \in \mathbb{R} : t\ge t_0 \}$ \\},% 
	sort={TimeSet}% 
]% 
{$\TimeSet$}
\newcommand{\TimeSet}{\Omega_{\sss{t_0}}}

% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %

\newterm 
[% 
	label={CurvatureSetEpsilon}, % label 
	description={$
							\Omega_{\kappa}^{{\tiny\dx}}(\epsilon) =
							\{
								\kappa \in \mathbb{R}_0^{+} :
								|\kappa \dx| <1-\epsilon^2,
								\epsilon \in \SetOne
							\}
						$\\},% 
	sort={TrimmingPathA}% 
]% 
{$\kLSetEpsilon$}
\newcommand{\kLSetEpsilon}[1][\epsilon]{\Omega_{\kappa}^{{\tiny\dx}}(#1)}

\newterm 
[% 
	label={CurvatureSet}, % label 
	description={$
							\Omega_{\kappa}^{{\tiny\dx}} =
							\{
								\kappa \in \mathbb{R}_0^{+} :
								(\kappa \dx)^2 <1 
							\}
							\equiv
							\Omega_{\kappa}^{{\tiny\dx}}(0)
						$\\},% 
	parent ={CurvatureSetEpsilon},
	sort={TrimmingPathB}% 
]% 
{$\kLSet$}
\newcommand{\kLSet}{\Omega_{\kappa}^{{\tiny\dx}}}

\newterm 
[% 
	label={TrimmingPathEpsilon}, % label 
	description={Trimming path, i.e. \\
	$
		\Omega_{\sss{\text{TP}}}^{{\tiny\dx}}(\epsilon) =
		\{
			\bm{\kappa}=\tau \eOne+ \kappa \eThree,
			\kappa \in \mathbb{R}_0^{+},
			\tau \in \mathbb{R}
			:
			\forall_{t \in \TimeSet}  \dot{\bm{\kappa}}(t)=\zvec
			\wedge
			\kappa \in \kLSetEpsilon
		\}
	$\\},% 
	sort={TrimmingPathC}% 
]% 
{$\TrimSetEpsilon$}
\newcommand{\TrimSetEpsilon}[1][\epsilon]{\Omega_{\sss{\text{TP}}}^{{\tiny\dx}}(#1)}

\newterm 
[% 
	label={TrimmingPath}, % label 
	description={Trimming path, i.e. \\
	$
		\Omega_{\sss{\text{TP}}}^{{\tiny\dx}} =
		\{\bm{\kappa}=\tau \eOne+ \kappa \eThree,
		\kappa \in \mathbb{R}_0^{+},
		\tau \in \mathbb{R}
		:
		\forall_{t \in \TimeSet}  \dot{\bm{\kappa}}(t)=\zvec
		\wedge
		\kappa \in \kLSet\}
		\equiv \TrimSetEpsilon[0]
	$\\},% 
	parent ={TrimmingPathEpsilon},
	sort={TrimmingPathD}% 
]% 
{$\TrimSet$}
\newcommand{\TrimSet}{\Omega_{\sss{\text{TP}}}^{{\tiny\dx}}}

\newterm 
[% 
	label={TrimmingNonPathEpsilon}, % label 
	description={Non-Trimming path, i.e. \\
	$
		\Omega_{\sss{\text{NTP}}}^{{\tiny\dx}}(\epsilon) =
		\{
			\bm{\kappa} =\tau \eOne+ \kappa \eThree,
			\kappa \in \mathbb{R}_0^{+},
			\tau \in \mathbb{R}
			:
			\exists_{t \in \TimeSet}  \dot{\bm{\kappa}}(t)\ne\zvec
			\wedge
			\kappa \in \kLSetEpsilon
		\}
	$\\},% 
	sort={TrimmingPathE}% 
]% 
{$\NonTrimSetEpsilon$}
\newcommand{\NonTrimSetEpsilon}[1][\epsilon]{\Omega_{\kappa}(#1)}

\newterm 
[% 
	label={TrimmingNonPath}, % label 
	description={Non-Trimming path, i.e. \\$
		\Omega_{\sss{\text{NTP}}}^{{\tiny\dx}} =
			 \{
				 \bm{\kappa}=\tau \eOne+ \kappa \eThree,
				 \kappa \in \mathbb{R}_0^{+},
				 \tau \in \mathbb{R}
				 :
				 \exists_{t \in \TimeSet}  \dot{\bm{\kappa}}(t)\ne\zvec 
				 \wedge
				 \kappa \in \kLSet
			 \}
			 \equiv
			 \NonTrimSetEpsilon[0]
	$\\},% 
	parent ={TrimmingNonPathEpsilon},
	sort={TrimmingPathF}% 
]% 
{$\NonTrimSet$}
\newcommand{\NonTrimSet}{\Omega_{\sss{\text{NTP}}}^{{\tiny\dx}}}

% ------------------------------------------------------------------------------ %
% ------------------------------------------------------------------------------ %

\newterm 
[% 
	label={SetOne}, % label 
	description={$\Omega_1 = \{x \in \mathbb{R}=  |x| \le 1\}$\\},% 
	sort={SetA}% 
]% 
{$\SetOne$}
\newcommand{\SetOne}{\Omega_1}

\newterm 
[% 
	label={SetTwo}, % label 
	description={$\Omega_2 = \{x \in \mathbb{R}=  0 \le x \le 2\}$\\},% 
	sort={SetB}% 
]% 
{$\SetTwo$}
\newcommand{\SetTwo}{\Omega_2}

==> SetUps/Units.tex <==
% units

% velocity
\newcommand{\velUnit}{\frac{\text{m}}{\text{s}}}

% seconds
\newcommand{\secUnit}{\text{s}}

% meters
\newcommand{\metUnit}{\text{m}}
